Interactive Diversity Optimization of Environments

The design of a building requires an architect to balance a wide range of constraints: aesthetic, geometric, usability, lighting, safety, etc. At the same time, there are often a multiplicity of diverse designs that can meet these constraints equally well. Architects must use their skills and artistic vision to explore these rich but highly constrained design spaces. A number of computer-aided design tools use automation to provide useful analytical data and optimal designs with respect to certain fitness criteria. However, this automation can come at the expense of a designer's creative control. We propose uDOME, a user-in-the-loop system for computer-aided design exploration that balances automation and control by efficiently exploring, analyzing, and filtering the space of environment layouts to better inform an architect's decision-making. At each design iteration, uDOME provides a set of diverse designs which satisfy user-defined constraints and optimality criteria within a user defined parameterization of the design space. The user then selects a design and performs a similar optimization with the same or different parameters and objectives. This exploration process can be repeated as many times as the designer wishes. Our user studies indicates that \DOME, with its diversity-based approach, improves the efficiency and effectiveness of even novice users with minimal training, without compromising the quality of their designs.

==> tex/fancey/highlighting_lib.tex <==


\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
        }

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}

==> tex/project_Analysis.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[trim={3.5cm 8.5cm 4.5cm 8.5cm},clip, width=0.4\textwidth]{../images/cpugpu1.pdf}
	\caption{CPU and GPU total graph construction and metric computation time comparison on an example environment. It is evident that the GPU ported version completes the computation much faster, for example at around 1000 nodes the GPU takes 58ms compared to CPU's ​280ms. The differece becomes much more substantial as the number of nodes in the graph increase. Note that this test compares a very high-end CPU with average commercial GPUs. The solid line is the average over 10 runs, with dashed lines showing two standard deviations above and below the average.}
	\label{figure:cpugpu}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[trim={4cm 8.5cm 4.5cm 8.5cm},clip, width=0.4\textwidth]{../images/metrics_sens.pdf}
	\caption{Sensitivity of metric values to sampling frequency, averaged over a variaty of environment. Vertical axis value is the average standard deviation of metric value taken over a window of size 5 around the given sampling frequency, averaged over several different environment. These diagrams show how the metric values do not substantially change after a certain point in sampling frequency, suggesting that a "good enough" value can be selected for the sampling frequency. Note that the two jumps in the depth and entropy diagrams are caused by discovering new bottlenecks after a certain increase in granularity of the environment, which are discarded at higher sampling frequency. Thus a much lower frequency is good enough.}
	\label{figure:metrics_sens}
\end{figure*}

\section{Metrics Analysis}

\subsection{Sensitivity Analysis}

\subsection{GPU Analysis}


==> tex/project_Curvature.tex <==


\section{Discrete Curvature on a Mesh}
\label{sec:curvature}

% \reviewerCommant{equations 1-3 assume that the curve is arclength parameterized.}

Briefly the calculations for both 2D and 3D discrete curvature are reviewed below and a description of the specific curvature formulation in is described the following section. 

\begin{figure}[htb]
	\includegraphics[width=0.95\linewidth]{../images/osculating_circles.pdf}
	\caption{\label{figure:2dline} A 2D parametric curve with two osculating circles that illustrate the curvature at points $s_{0}$ and $s_{1}$.}
\end{figure}

\subsection{Curvature in 2D}

% \reviewerCommant{it should be arc length parameterization for the equations before Equation 5}

Given a parametric 2D curve  $\paramLine = (\paramLineX,\paramLineY), 0 \leq s \leq $ curve length, the differential concept of curvature, $\curvature$, is defined as follows:
\begin{eqnarray}
	& & \paramTangent = \paramLinePrime \label{equ:line-tangent} \\
	& & \paramTangentPrime = \paramLinePrimePrime = \curvatureSigned \paramNormal \label{equ:line-acceleration} \\
	& & 	\curvature = ||\paramTangentPrime|| = ||\paramLinePrimePrime|| =  |\curvatureSigned|  \\ % = |\differential\paramTangent \label{equ:line-curvature} \\
	& & \paramRadius = \curvature^{-1}, \label{equ:line-circle-radius}
\end{eqnarray}
where \paramTangent is the tangent vector, and \paramNormal is the unit normal vector that points towards the centre of the inscribed circle with radius \paramRadius. Figure~\ref{figure:2dline} shows the osculating circles with the radii in solid blue for two points on the curve. The signed curvature is computed independently of the derivative's magnitude as follows:
\begin{equation}
	\curvatureSigned = \frac{\paramLineXPrime \paramLineYPrimePrime - \paramLineYPrime \paramLineXPrimePrime}{(\paramLineXPrime^{2} + \paramLineYPrime^{2})^{3/2}}.
\end{equation}

%\petros{ Are you saying that the (x',y') is normalized?  -- This uses the unit length tangent to compute the signed curvature independent of the derivative magnitude.}
%\glen{The tangent is normalized to unit length, so yes.}


\subsection{Curvature of a Surface}

% \reviewerCommant{Description in 3.2 is inaccurate, e.g., "where kappa\_max points in the direction of the maximal curvature..." but kappa\_max is a scalar, it is really just the maximum curvature.}

% The concept of curvature extends to three dimensions. 
% Many features of curvature in two dimensions extend to three dimensions. 
Let \surface be a surface embedded in \Rthree, where points on the surface are defined by the parametrization \paramSurface.
The normal of the tangent plane can be computed from the cross product of the parametric derivatives:
%The tangent plane can be calculated from the partial derivatives of the parametrize surface \paramSurface as
%\begin{equation}
%	\frac{\partial\paramSurface}{\partial\surfaceParamU} , \frac{\partial\paramSurface}{\partial\surfaceParamV},
%\end{equation}
%\noindent
%With the plane normal as 
\begin{equation}
	\paramSurfaceNormal = \frac{\partial\paramSurface}{\partial\surfaceParamU} \times \frac{\partial\paramSurface}{\partial\surfaceParamV}
\end{equation}
	
For every unit direction $\vectore_{\direction}$ in the tangent plane, the \emph{normal curvature} $\normalCurvature(\direction)$ is the curvature of the plane in the direction $\vectore_{\direction}$ at point $(\surfaceParamU,\surfaceParamV)$. 
The  \emph{principal curvatures} of the surface, $\vec{\Kmax}$ and $\vec{\Kmin}$, correspond to orthogonal directions on the tangent plane. Where $\vec{\Kmax}$ points in the direction of the maximal curvature and $\vec{\Kmin}$, the minimal curvature of $\normalCurvature(\direction)$.
% These are not necessarily in the same direction as the partial derivatives.
Calculating the principal curvatures is non-trivial, particularly on a discrete surface and is a large area of research. 
The normal curvature, \normalCurvature(\direction) is sometimes expressed in terms of the two principal directions as
\begin{equation}
	\normalCurvature(\direction) = \vec{\Kmax}  \cos^{2}(\direction) + \vec{\Kmin} \sin^{2}(\direction).
\end{equation}
$\Kmax$ and $\Kmin$ are equal to the magnitudes of their vector form.

% \reviewerCommant{where did equation 7 come from? In particular it requires that theta=0 be the principle direction of largest curvature.}


\noindent\textbf{Mean Curvature} is the average curvature over all directions \direction, at a point on a surface, which can be expressed in terms of the normal curvature \normalCurvature(\direction), or the average of the principal curvatures:
\begin{eqnarray}
\meanCurvature &= \dfrac{1}{2\pi} \int_{0}^{2\pi} \normalCurvature(\direction)  d\direction \\\nonumber
	&= \dfrac{1}{2}(\Kmin + \Kmax).
\end{eqnarray}
\noindent
The next section presents the discrete form of mean curvature that is use in the analysis. 

\subsection{Discrete Mean Curvature}

A mesh is a discrete approximation of a surface in 3D. 
% To calculate curvature on a mesh approximations are used.
The mesh representation in practise is made up of many \faces that may have discontinuities at every edge. 
To cope with the mathematical issues of dealing with discontinuities, each edge is understood as being uniformly round. 
% This makes a framework for curvature calculations at edges and \vertices. 
The mean curvature is calculated at \vertices on a polygonal mesh following~\cite{diffGeoOps}. 
For completeness, the main formulae involved are presented. 

The mean curvature normal is computed via the gradient of the area around the \vertex \vectorx.
\begin{equation}
	\int\int_{\Area} \textbf{K}(\vectorx)  d\Area = \nabla \Area_{1-ring}
\end{equation}
The equation from which the mean curvature at a \vertex is calculated is then
\begin{equation}
	\int\int_{\Area} \textbf{K}(\vectorx_{i})  d\Area = \frac{1}{2} \sum_{j\in N(i)}^{}(\cot(\alpha_{ij}) + \cot(\beta_{ij})) (\vectorx_{i}-\vectorx_{j}),
\end{equation}
%\captionsetup[figure]{labelfont=scriptsize}
\noindent 
% \petros{ $k^H $ is constant, isn't it?}  
where $N(i)$ is the 1-ring of neighbour \vertices around \vertex $i$,   and $\alpha_{ij}$ and $\beta_{ij}$ are the angles subtended by the common edge of the two adjacent \faces, Figure~\ref{figure:small-triangles}. 
The surface area, $\Area$, is computed using a \emph{Voronoi} region approach, however it suffers from numerical issues when the triangles have obtuse angles.  To address these issues the surface area $\Area$ of $N(i)$ is compute the as the sum of area estimates for all triangles in the 1-ring as follows. 
For each non-obtuse triangle the \emph{Voronoi} area  \voronoiArea is added and for each obtuse triangle either half or a quarter of the triangle area is added. 
 % by combining the \emph{Voronoi} area \voronoiArea and the \glen{\emph{Barycentric} area \barycentricArea}.  
The \emph{Voronoi} area \voronoiArea is defined as:
	\begin{equation}
		\voronoiArea = \frac{1}{8} \sum_{j\in N(i)}^{}(\cot(\alpha_{ij}) + \\ \cot(\beta_{ij})) ||\vectorx_{i}-\vectorx_{j}||^{2}
	\end{equation}
%\glen{and the \barycentricArea is a third of the area of the area of the 1-ring of neighbours}

  This approach  results in a mixed formulation for  \Area denoted as \mixedArea.  For more details please see~\cite{diffGeoOps}.
  
  The final formulation for the discrete mean curvature that is used in this work is 
 \begin{equation}
 \meanCurvatureVec(\vectorx_{i}) = \frac{1}{2\mixedArea} \sum_{j\in N(i)}^{}(\cot(\alpha_{ij}) + \cot(\beta_{ij})) (\vectorx_{i}-\vectorx_{j}),\\
\end{equation}
\noindent with magnitude
 \begin{equation}
 \meanCurvature(\vectorx_{i}) = \frac{1}{4\mixedArea} \sum_{j\in N(i)}^{}(\cot(\alpha_{ij}) + \cot(\beta_{ij})) (\vectorx_{i}-\vectorx_{j}) \cdot {\bf n},\label{eq:finalcurvature}
\end{equation}
\noindent
where ${\bf n}$ is the normal vector.

\begin{figure}
%	\begin{wrapfigure}{r}{0.15\textwidth} % controls margin around figure
%		\vspace{-15pt}
		\begin{center}
		\includegraphics[width=0.15\textwidth]{../images/cotan-diagram.pdf}
		\end{center}
		%		\setbeamerfont{figure:small-triangles}{size=\scriptsize}
%		\caption{\scriptsize\label{figure:small-triangles}2 adjacent triangles}
\caption{\label{figure:small-triangles} The 1-ring neighbourhood of vertex $\vectorx_{i}$ and the cotangent angles for an edge $\langle \vectorx_{i}, \vectorx_{j} \rangle$.}
%	\end{wrapfigure}
\end{figure}	
%Angles $\alphas$ and $\beta$ can be seen in Figure~\ref{figure:small-triangles}.
	% This is equivalent to the gradient at $i$.
	
%\captionsetup[figure]{labelfont=normalsize}
% \reviewerCommant{although the formulation of mean curvature as the area gradient is very elegant, unless the mesh is nicely-shaped the result is not always very accurate. At the risk of being accused of heresy, I recommend using iterated quadratic fitting to estimate mean curvature, which is messier but more accurate particularly on coarse, noisy meshes.}

==> tex/project_Features.tex <==


\subsection{Iterative Design Process}


The user interaction process is meant to be iterative. 
An initial architecture can be created or loaded from a file.
Once a rough architectural design is prepared a user can select architectural elements that the user believes could be better placed but is unsure what this better placement might be.

\todo{This will be replaced with a figure}
\begin{enumerate}
	\item The user starts with no architecture or load some already created structure that the user may want to alter.
	\item The user can select any element in the environment to be optimized.
	When an item is selected the user selects translational or rotational bounds that the user would find acceptable for element to change.
	These bounds will be inserted into the optimization as hard constraints.
	\item The user can also select groups of elements at a time. 
	This group will be translated or rotated together during optimization.
	\item In order to facilitate a very robust method of adding bounds to element(s) from an architectural design of a building we embed the architectural layout in a \architecturalGraphText.
	This organizational structure allows us to alter the configuration of items in the environment while respecting many of the original architectural design features.
	For example, if optimizing the location of one portion of an L-shaped wall we want to keep the two walls joined together.
\end{enumerate}

The steps involved and the process controlled by the user is illustrated in Figure~\ref{figure:interaction-process}.

\begin{comment}
\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{../images/InteractionProcess.pdf}
\caption{\label{figure:interaction-process} The process flow for user interaction.}
\end{figure}
\end{comment}


\subsection{Examples}




==> tex/project_Metrics-ignore.tex <==
\begin{comment}
Any urban structure is built with several purposes in mind, most of which are directly related to the people who will use these structures. People's behaviour in an environment is mostly governed by two main factors: human spatial cognition, and the environmental elements \todocite{}. Considering the human spatial cognition as a fixed model, we seek to analyze the spatial relationship between environment elements and its impact on human behaviour. For example, certain placements of pillars can affect the evacuation speed of an environment \todocite{}, positioning of navigational signs in a building greatly affects how people navigate towards their goals \todocite{}, specific wall arrangements can hugely affect the attention directed towards specific parts of the environment, etc.

To analyze an environment, we need to formulate certain behaviours of interest into computable features. There are two possible approaches to this formulation: static feature formulation and dynamic feature formulation. The former, formulated in environmental design research as {\ssx}, calculates features based only on the position of environmental elements and argues that such features comply with certain real-life human behaviours (through real-life experiments) \todocite. The latter, known as \emph{Crowd Simulation}, computes features by modelling human behaviour into virtual agents which will then occupy the environment in a computer simulation, providing results and arguing that the results are as accurate as the human modelling. In this work, we only focus on {\ssx} as a well researched method, which can provide reliable insights and features about the environment \todocite{}.
\end{comment}

% \todo{To waste space in order to avoid compile error with reference spanning across two pages.}

% It has been shown that people's behaviour in an environment is governed by two factors: human spatial cognition, and the environmental elements~\cite{hillier2006studying,holscher}.
% Considering the human spatial cognition as a fixed model, we seek to analyze the spatial relationship between environment elements and its impact on human behaviour. For example, certain placements of pillars can affect the evacuation time of an environment~\cite{berseth2015environment}, positioning of navigational signs in a building greatly affects how people navigate towards their goals~\cite{holscher}, specific wall arrangements can hugely affect the attention directed towards specific parts of the environment, etc.


\ignore{
\textbf{Visibility Graph.} A graph where each vertex represents a point in the space, and each edge represents the visibility between two points. Points A and B in space are visible with respect to each other if and only if the straight line connecting them does not pass through any obstacle. In this sense, visibility is a binary variable for each two points in space. A visibility graph is constructed, in either two or three dimension, based on an underlying grid decomposition of the space which determines the potential vertices that can be included in the graph. Once a visibility graph is constructed for an environment, several graph features can be analysed such as vertex/edge connectivity, mean depth, shortest path, etc. and be considered as static metrics for describing that environment.

\textbf{Axial Map.} An axial map is defined as the minimal set of the fewest and longest lines of sight that cover some set of the widest convex spaces in terms of their area to parameter ratio. This definition can not be easily implemented, therefore an alternative definition is used: all longest lines of sight that cover the convex spaces are considered. After this decomposition, a graph is generated with each vertex representing one axial line and each edge representing the intersection of two axial lines. Using the generated axial graph, same analysis as the previous part can be conducted.
}

\begin{comment}
Then separate regions of the environment can be selected to be included as the graph vertices. Each selected region is be decomposed into points located at the center of grid cells encompassed by the region. However building a visibility graph over all the added regions is not the most useful construction. Suppose we want to maximize the degree of a visibility in a specific area in an environment, for example a specific event in an art gallery, or a fire exit door. So we have an area over which we want to measure degree, however this task inherently requires a definition of some reference: "with respect to which areas we want the painting region to be more visible (integrated)?" or "with respect to which areas we want the exit sign to be more visible?". The answer to such questions may be "the whole environment", "entrance doors", "a specific hall", and so on. So merely constructing the visibility graph over the whole environment, as is often done in {\ssx} is not the most informative way of decomposition.
\end{comment}

%This new form of representing the {\ssx} increases the range of questions that can be answered by static environment analysis, and provides unique information tailored to each specific task.


%Figure~\ref{figure:metrics}d shows the degree of visibility computed over the {\roq} with respect to {\ror} which is shown in yellow. Notice how changing the reference from the entire environment in part a, to just the top and bottom hallways can greatly affect the computed values, and therefore changes any optimization task. Same effect is in place for the other two metrics. This new form of representing the {\ssx} increases the range of questions that can be answered by static environment analysis, and provides unique information tailored to each specific task.


\begin{comment}
\textbf{\roq.} The set of all nodes that are to be considered as objective targets, that is the nodes over which we the average spatial analysis measures. These points are considered as separate vertices in the graph, not connected to each other, but only connected to {\ror} vertices. You can think of this as each {\roq} vertex having a separate graph of its own, consisted of that vertex and all the {\roq} vertices.
\textbf{\ror.} the union of all the points that are considered as reference for calculating the objective, that is the points with respect to which the metrics are calculated. These vertices can have edges between themselves and query region vertices.

\begin{equation}
\visibilityGraph = \phi (\nodesN_r,\nodesN_q, \architecturalGraph(P), d)
\end{equation}

\end{comment}



\ignore{
however we focus on the degree of each node in the graph, as it is one of the most widely used and informative features in the \spaceSyntaxText community. The degree of each node in a visibility graph shows the number of visible points in the space from the point of view of that node. This degree number basically represents the complete field of view of each node: the higher the degree, the more visible the node. Intuitively, this can be interpreted as the attention one node (one point in space) gathers from the surrounding environment, and therefore increasing the degree of a node results in that node being more easily accessible. This notion of visibility can be in fact of paramount importance in environments: increasing the visibility of exit doors may facilitate evacuation during emergencies, while  increasing the visibility of a certain point can draw more people towards it (e.g. a sign, a painting, an important section, etc.). It is generally accepted in various communities that  increasing the overall visibility of an environment has often both aesthetic and practical advantages.

% makes is easier to traverse. Note that while many of these results are merely intuitive and lack solid proofs, several real-life experiments in the \spaceSyntaxText community do in fact confirm much of the mentioned conclusions (cite).

%Therefore, we will consider the node degree, or average node degree of several points of interest, in the visibility graph as the feature for analysis and eventually optimization. Local and global degree can be maximized or minimized in order to increase or decrease visibility/accessibility of one or several points respectively.

Therefore, we will consider the node degree of the visibility graph as the main feature for analysis and optimization. Our experiments  most often involve average node degrees computed for appropriate groups of nodes.   
}


\ignore{
\subsection{Dynamic Analysis: Crowd Simulation}

In contrast to static techniques, crowd simulation can be used as an alternative method that  offer insights about the traversability, connectivity and other aspects of an environment. Crowd simulation models the dynamic behaviour of a crowd, and thus can provide information  about the interaction between agents and the environment that is time-dependent. Furthermore, it can explicitly model non-homogeneous properties of a crowd, such as disabilities, varying relationships between agents, and different roles (civilians, emergency personnel, etc.).  

The effectiveness of crowd simulation  is predicated on the fidelity of the simulated results to  real crowd behaviour. Although, many methods have been developed to simulate crowds \cite{}, there is no widely accepted approach that is proven to mimic a wide range of real crowd behaviours. Nevertheless, it is a widely used  alternative which can serve as a basis of comparison with our analysis. In the future, we plan to explore a space analysis method that combines both approaches. 

\subsection{Dynamic Analysis: Crowd Simulation}
In crowd simulation, first a model is considered and tuned to mimic the behaviour of humans in a given environment. Then, a crowd govern by this model occupies a virtual environment (generated based on the plan of a real environment), which is analysed and interpreted to achieve some features such as flow of people in the environment. These features correspond to how a real human crowd would behave as long as the modelling process is justified.
Several crowd models have been explored in the crowd simulation community, most notably PPR, SF and ORCA, each having specific parameters and providing certain characteristics of real human crowds (cite). Also, these models' parameters can be tune towards certain effects, highlighting some specific features (cite).

Dynamic analysis, based on crowd simulation, can in theory become far more accurate in comparison to static \spaceSyntaxText approach. \spaceSyntaxText is limited because of the fact that its analysis is intrinsically based on calculating heuristic features, and then assuming connections between these features and the actual human behaviour, which may not be able to exceed some point of accuracy. However, the computation overhead of crowd simulation limits the dynamic approach as well. So the best approach would be a combination of these approaches, where \spaceSyntaxText calculates some features and which are then fine-tuned by crowd simulation.

In this work, we will only use dynamic analysis in order to provide a basis of comparison for \spaceSyntaxText results. The fusion of the two approaches will be subject of future works.
}

%The degree of visibility is representative of how integrated a region is in an environment, i.e. how much attention a region attracts. The more the degree of visibility for a point, the better its field of view in the environment, and consequently increased attention and crowd attraction is expected for the point. Figure~\ref{figure:metrics}  shows the computed degree values in a heat map form over a sample environment. In this toy example, see how center-left region and right-side corners show very high degree of visibility compared to the points within the upper and lower corridors. This suggests that those areas are much more integrated in the environment, will face more crowd density and are potentially good candidates for placement of important features (e.g. fire exits, signs, main events, etc.). This information provides very important insight to a designer, and utilizing this information can potentially affect the efficiency of an environment to a great extend.

\begin{comment}
The regions of interest provide the user with great flexibility. 
% subject to $\exists e(v_i,v_j) \not \in \Eg: v_i,v_j \notin \V_r$, that is the {\roq} vertices can only be connected to the {\ror} vertices (note that the two sets can share points).
This condition provides the user with all possible choices in region selection, for example a user can choose to include the {\roq} in selection of the {\ror} to investigate inner relationship of target regions, or can exclude the {\roq} to only focus on the cross relationships with the reference regions. The resulting visibility graph is a function of these two \textit{user-specified} regions, in addition to the architectural graph and the sampling grid $V$:
\begin{equation}
\visibilityGraph = \phi (\gridNodes_r,\gridNodes_q, \architecturalGraph(\vectorParameters), V)
\end{equation}
%We compute the metrics only for the nodes of the  {\roq}.

We provide the selection of regions of reference and query as optional interaction steps for designers using our tool for space analysis, with default values spanning the entire environment. 
\todo{This increases the range of space analysis questions that one can ask, allowing designers to focus their analysis on specific aspects of the layout.}\glen{Yes this is great! This is why we have these. It should be noted earlier to motivate this stuff.}
  
\end{comment}  



==> tex/project_Navmesh.tex <==
	



==> tex/project_glosary.tex <==
\section{Glossary}
Glossary of terms to keep consistent while writing
\begin{enumerate}
	\item Use British/Canadian english spelling
	\item node \node is for the \architecturalGraphText
	\item $q_{i}$ are the \architecturalGraph parameters
	\item $\vectorParameters$ are the optimization parameters
	\item vertex is for the visibility graph
	\item main event $\rightarrow$ focal point
	\item Use "\textbackslash reffig" instead of "Figure \textbackslash ref". It produces Fig. i.
	\item we should give less "For examples"....
	\item motivate sections and paragraph early. Doing it later makes me uninterested in the writing, I want to skip it. We need to give them a reason to want to read the text, every word...
	\item Need to reduce the amount of adjectives used. It makes the writing sound less scientific and more opinionated.
	\item for function names italic and first letter of word is capital.
	\item use the work "method" to describe \DOME (not approach or framework, etc...)
	\item when referring to the current design being worked on use the word "environment" not layout, building, etc...
\end{enumerate}
